Examining Temporalities on Stance Detection towards COVID-19 Vaccination

Previous studies have highlighted the importance of vaccination as an effective strategy to control the transmission of the COVID-19 virus. It is crucial for policymakers to have a comprehensive understanding of the public's stance towards vaccination on a large scale. However, attitudes towards COVID-19 vaccination, such as pro-vaccine or vaccine hesitancy, have evolved over time on social media. Thus, it is necessary to account for possible temporal shifts when analysing these stances. This study aims to examine the impact of temporal concept drift on stance detection towards COVID-19 vaccination on Twitter. To this end, we evaluate a range of transformer-based models using chronological (splitting the training, validation, and test sets in order of time) and random splits (randomly splitting these three sets) of social media data. Our findings reveal significant discrepancies in model performance between random and chronological splits in several existing COVID-19-related datasets; specifically, chronological splits significantly reduce the accuracy of stance classification. Therefore, real-world stance detection approaches need to be further refined to incorporate temporal factors as a key consideration.

==> reviews.tex <==
1: (weak accept)
This paper studies whether performance of classifiers for stance detection towards COVID-19 vaccination degrades when training and testing time periods do not align. The authors experiment with five datasets (3 English, 2 multilingual) and five models (BERT, COVID BERT, VAXX BERT for English, XML-BERT, XML-RoBERTa for multilingual). They study differences in performance on Random and Chronological splits, and also look at how accuracy correlates with overlap of tokens in the training and test sets.

Strengths:
* The choice of problem is very good, as I would expect to see significant temporal drift in how vaccines are discussed. The results are therefore unsurprising but still interesting!
* The author's setup for classification follows a fairly standard procedure, and the setup of chronological vs. random splits is well thought-out.

Weaknesses:
* I think that there is a logical jump in the Discussion for Q3. The authors go from saying that domain adapted PLMs outperform vanilla BERT on monolingual datasets to saying that appllying domain/task adaptation can address temporal concept drift. However, it seems as though to prove this point, the authors should directlly compare the *difference* in scores between the random and chronological splits, which the wording implies is not necessary. It is possible to do this from the Table in the paper, which largely supports the authors conclusion, but difficult to do manually. The authors might consider another way of presenting this information.
* The results seem somewhat overstated when the difference between random and chronological splits is only statistical significant for 2/5 datasets.
* The framing could be improved. The authors use the word "overestimation" to discuss the results using random splits. This implies overestimation in a specific use case, e.g., trying to apply a model that was trained on past data to current data, but this is not really discussed.

Minor comments/questions:
* For a reader who is unfamiliar with this area of work, the meaning of chronological/random splits might be unclear in the abstract.
* I think a citation should be given for the DICE coefficient.
* The discussion for Q3 could have a reference to Table 2.
* The authors mention that the models are tuned on the validation set. What parameters are tuned? The authors only share their final learning rate/batch size/max input tokens.
* Could there be overlap between the data that Vaccine-BERT is trained on and your data? How might that affect the results?
* Is it correct that the authors only use different random seeds for chronological splits, but not for random splits? Could seeding the classifiers make a difference for the random splits?
* Did the authors consider using a measure related to time between training and test data instead of UoU/DICE?


---------------------------


2: (accept)
**Summary**

This paper researches how temporal concept drift influences stance classification results. Additionally, it analyzes how domain adaptation (e.g. more COVID-specific BERT models) as well as a setting in multiple languages influence classification performance. It also analyzes whether there is a semantic difference between the training and test set(s). Its experiments cover 5 datasets and 5 models, in two scenarios: chronological train-test splits, and random train-test splits.

**Strengths**

- This paper has solid research goals, sets up a clear experimental procedure, and evaluates the results based on earlier hypotheses (e.g. that more specific COVID-related models would have improved classification performance).

- The paper uses several datasets and several models, which more clearly show whether the results are (merely) a one-dataset trend.

- The use of significance testing to determine whether the difference in results across experimental paradigms is a meaningful difference or not.  


**Weaknesses / Possible Improvements**

- Are VaccineBERT and CovidBERT trained on the same datasets used in the experiments of this study? If this is the case, that would influence the results of this study: it may be less about domain-specificity, and more about memorization or at least highly specific pre-training. Mentioning the specific dataset used for pre-training these models would make this clear.

- The examples in the error analysis could be more specifically explained. What is meant with an “emerging topic”: is this a topic not in the training data but in the test-set? And why would this be more difficult for a chronological model rather than a model trained with random splits? The example mentioned is also not very clear to what is emerging about this: is this a topic coming up at a specific time in the timeline? While the cross-topic and emerging topic aspect is not part of the research questions, it seems to be quite prominent influence in the results.

- Additionally, the paper could make explicit which timeslots or emerging topics are difficult to generalize from. Is there a pattern to be found there?

- Will the code repository be available to aid the reproducibility of the experiments?

- The paper misses some key stance detection references, as well as a definition of the task by citing a core work. Adding these would embed the results better in the argument mining/stance detection field. Such a work could be "Stance Detection: A Survey" by Kucuk & Can, as well as "Argument Mining" by Laurence & Reed. Additional results on the brittleness of argument mining results is also missing, with one core recent example being "Stance Detection Benchmark: How Robust is Your Stance Detection?" by Schiller et. al. (2021), who show results are not consistent over multiple datasets and very vulnerable to simple pertubations. Adding this literature would give more context to the results.



**Clarity:**

- It would be helpful if the specific languages in the multi-language settings were mentioned, or at least (in the case of the 100+ language dataset) the most prominent languages in this dataset. Additionally, specifying these languages with A language tag from BCP-479 identifying the language variety, as specified in Bender & Friedman (2018)’s Data Statements paper.

- The paper would improve in clarity of the research line if it was more explicit in research questions: Q3 talks about the “impact” of temporal concept drift, I think “impact on (stance) classification performance” is more precise.

- The same with the word “discrepancy” in Q4: the semantic discrepancy is meant, what I gather from later sections: a discrepancy in which tokens/vocabulary are present. The same counts for the explanation of “similarity” and “variation” in the methods section: I think semantic variation is meant, but not made explicit.


\* Clarity of information in Table 2: The information in this table would be clearer if:

- differences in P/R/F1 between chronological and random were explicitly mentioned in a row below the two scores;

- These differences showed whether or not there was a significant difference. Significance can also be denoted with \* rather than a grey cell.

- The biggest difference can be denoted with a bolded score/number, to immediatley show a pattern of highest difference.

- Perhaps organizing the information in a graph, especially for the chronological splits, which would be able to show whether a chronological trend over time is visible across datasets.


**Conclusion/Summary**

This paper clearly states its research goals, and shows some interesting results for the time-dependency of stance classification results. Some edits with regards to references, specifics of the experiments and results, as well as some clarification in writing, would make the paper more solid and publishable.


----------------------------------------

2: (accept)
This paper discusses some interesting results in stance detection of COVID19 related tweets across languages and find that the performance of models degrades when testing on a time period different from the tweets in the training set. Overall, this is a useful contribution and fits the theme of the data challenge very well. For future work, I would suggest contextualizing the current work in research about time and NLP (see for example Loureiro, Daniel, et al. "Timelms: Diachronic language models from twitter." arXiv preprint arXiv:2202.03829 (2022).).
